Time-Varying ALIP Model and Robust Foot-Placement Control for Underactuated Bipedal Robot Walking on a Swaying Rigid Surface

Controller design for bipedal walking on dynamic rigid surfaces (DRSes), which are rigid surfaces moving in the inertial frame (e.g., ships and airplanes), remains largely uninvestigated. This paper introduces a hierarchical control approach that achieves stable underactuated bipedal robot walking on a horizontally oscillating DRS. The highest layer of our approach is a real-time motion planner that generates desired global behaviors (i.e., the center of mass trajectories and footstep locations) by stabilizing a reduced-order robot model. One key novelty of this layer is the derivation of the reduced-order model by analytically extending the angular momentum based linear inverted pendulum (ALIP) model from stationary to horizontally moving surfaces. The other novelty is the development of a discrete-time foot-placement controller that exponentially stabilizes the hybrid, linear, time-varying ALIP model. The middle layer of the proposed approach is a walking pattern generator that translates the desired global behaviors into the robot's full-body reference trajectories for all directly actuated degrees of freedom. The lowest layer is an input-output linearizing controller that exponentially tracks those full-body reference trajectories based on the full-order, hybrid, nonlinear robot dynamics. Simulations of planar underactuated bipedal walking on a swaying DRS confirm that the proposed framework ensures the walking stability under different DRS motions and gait types.

==> excess.tex <==
% There are several advantages of controlling the angular momentum about the contact point (i.e., $L_A$) over the CoM velocity (i.e., $\mathbf{v}_{CoM}$):
% \begin{itemize}
%     \item $L_A$ provides more comprehensive information about the current walking status because it does not only include the linear velocity $\mathbf{v}_{CoM}$, but also the angular momentum of the CoM.
%     \item The derivative of $L_A$ only depends on the CoM position w.r.t the contact point for an under-actuated robot. This means $L_A$ will be weakly affected by the motor peak torque and other disturbances, such as the aggressive motion of a swing leg.
%     \item $L_A$ is invariant if the robot is walking on flat terrain without vertical velocity. On the contrary, the linear velocity $\mathbf{v}_{CoM}$ experiences a jump at the impact based on the impact model, which is always less accurate compared to the continuous model. Using angular momentum about the contact point can help to avoid the inaccuracy that is introduced by the impact model. 
% \end{itemize}


%For simplification purposes, we utilize the sinusoidal wave to represent the DRS motion.



% \begin{itemize}
%     \item Point S: position of the contact point on the DRS w.r.t the wolrd frame.
%     \item Point A: a fixed point that is coincident with the point S at any time in the world frame.
%     \item $\mathbf{p}_{CoM} = [x_c, z_c]\in\mathbb{R}^2$: robot's CoM position in the world frame
%     \item $\mathbf{p}_{SA}=[x_{SA}, z_{SA}]\in\mathbb{R}^2$: position vector from point S to A
% \end{itemize}



% where $\dot{x}_C$ and $\dot{z}_C$ are its horizontal and vertical components.

% := [x_{sc}, z_{sc}]^T\in\mathbb{R}^2
% Note that during regular bipedal walking, the angular momentum $L_{CoM}$ typically oscillates around zero~\cite{9560821}.
% This is because a bipedal robot's trunk is usually built to be substantially heavier than the limbs and the trunk is typically commanded to exhibit negligible angular movement w.r.t. the world frame.

% There are several advantages of controlling the angular momentum about the contact point (i.e., $L_A$) over the CoM velocity (i.e., $\mathbf{v}_{CoM}$)~\cite{9560821}:
% \begin{itemize}
%     \item $L_A$ provides more comprehensive information about the current walking status because it does not only include the linear velocity $\mathbf{v}_{CoM}$, but also the angular momentum of the CoM.
%     \item The derivative of $L_A$ only depends on the CoM position w.r.t the contact point for an under-actuated robot. This means $L_A$ will be weakly affected by the motor peak torque and other disturbances, such as the aggressive motion of a swing leg.
%     \item $L_A$ is invariant if the robot is walking on flat terrain without vertical velocity. On the contrary, the linear velocity $\mathbf{v}_{CoM}$ experiences a jump at the impact based on the impact model, which is always less accurate compared to the continuous model. Using angular momentum about the contact point can help to avoid the inaccuracy that is introduced by the impact model. 
% \end{itemize}
Both original LIP and ALIP suffer accuracy loss from increasing Lc, but ALIP preserves more accuracy as the legs get heavier.

Lc oscillates about zero but I don't think it is always small, Cassie, Digit, mini-cheetah, and Spot have light legs but many other robots have heavy legs. And the legs generate non-negligible Lc when walking.


    % Recently, locomotion on deformable surfaces has been increasingly extensively studied.
    % D. Goldman .et.al investigated the robot locomotion dynamics on granular terrain~\cite{aguilar2016robophysical,li2013terradynamics}. The granular terrain is considered a dynamic surface because the contact between the robot and the surface is subject to significant movement during any step.
    % Later, a model for granular terrain and stability criteria of such locomotion are proposed~\cite{xiong2017stability}, which can guide the control design for a legged robot walking on such terrain with guaranteed stability. 

    % Besides granular terrain, another type of dynamic surface also attracts research interest. Unlike the granular terrain, this type of dynamic surface does not deform but exhibits particular motion w.r.t the world frame. In a real-world application, this type of dynamic surface includes airplanes, ferries, and ground vehicles.
